Generalizing the intention-to-treat effect of an active control against placebo from historical placebo-controlled trials to an active-controlled trial: A case study of the efficacy of daily oral TDF/FTC in the HPTN 084 study

In many clinical settings, an active-controlled trial design (e.g., a non-inferiority or superiority design) is often used to compare an experimental medicine to an active control (e.g., an FDA-approved, standard therapy). One prominent example is a recent phase 3 efficacy trial, HIV Prevention Trials Network Study 084 (HPTN 084), comparing long-acting cabotegravir, a new HIV pre-exposure prophylaxis (PrEP) agent, to the FDA-approved daily oral tenofovir disoproxil fumarate plus emtricitabine (TDF/FTC) in a population of heterosexual women in 7 African countries. One key complication of interpreting study results in an active-controlled trial like HPTN 084 is that the placebo arm is not present and the efficacy of the active control (and hence the experimental drug) compared to the placebo can only be inferred by leveraging other data sources. \bz{In this article, we study statistical inference for the intention-to-treat (ITT) effect of the active control using relevant historical placebo-controlled trials data under the potential outcomes (PO) framework}. We highlight the role of adherence and unmeasured confounding, discuss in detail identification assumptions and two modes of inference (point versus partial identification), propose estimators under identification assumptions permitting point identification, and lay out sensitivity analyses needed to relax identification assumptions. We applied our framework to estimating the intention-to-treat effect of daily oral TDF/FTC versus placebo in HPTN 084 using data from an earlier Phase 3, placebo-controlled trial of daily oral TDF/FTC (Partners PrEP).

==> old_real_data.tex <==

%If Assumption 3 fails in Partners PrEP Study, $CATE(\mathbf{X}; S = h)$ can be partially identified by constructing partial identification intervals $[L(\mathbf{X}), U(\mathbf{X})]$ such that $CATE\left(\mathbf{X} ; S=h\right) \in[L(\mathbf{X}), U(\mathbf{X})]$ almost surely (see Remark 4). In this case, we can still obtain complier average treatment effect from the decomposition equation, but are only able to derive bounds of average treatment effect for always takers and never takers. The upper bound for $CATE(\mathbf{X};S= h; \text{always takers or never takers)})$ is 0 as we believe TDF/FTC is beneficial for HIV prevention. While the lower bound for $CATE(\mathbf{X};S= h; \text{always takers or never takers)})$ is $-\mathbb{E}[Y(Z=0)|S = h;\mathbf{X}]$ by taking $\mathbb{E}[Y(Z=1)|S = h; \mathbf{X}]$ as 0, which means no one would be infected with HIV after taking TDF/FTC. The empirical compliance rate is 0.728 in Partners PrEP Study, thus
$$
\begin{aligned}
L(\mathbf{X}) &= P(\text{compliers}; \mathbf{X}) \cdot CATE(\mathbf{X};S= h; \text{compliers}) + \left(1 - P(\text{compliers}; \mathbf{X})\right)(-\mathbb{E}[Y(Z=0)|S = h;\mathbf{X}])\\
&= \mathbb{E}[D(Z=1) - D(Z=0) |S = h; \mathbf{X}] \cdot \frac{\mathbb{E}[Y(Z=1) - Y(Z=0) | S = h; \mathbf{X}]}{\mathbb{E}[D(Z=1) - D(Z=0) |S = h; \mathbf{X}]} + \\
& \quad \quad \quad \quad \quad \quad \left(1 - \mathbb{E}[D(Z=1) - D(Z=0) |S = h; \mathbf{X}]\right)(-\mathbb{E}[Y(Z=0)|S = h;\mathbf{X}])\\
&= \mathbb{E}[Y(Z=1) - Y(Z=0) | S = h; \mathbf{X}] + \left(1 - \mathbb{E}[D(Z=1) - D(Z=0) |S = h; \mathbf{X}]\right)(-\mathbb{E}[Y(Z=0)|S = h;\mathbf{X}]),\\
\\
U(\mathbf{X}) &= P(\text{compliers}; \mathbf{X}) \cdot CATE(\mathbf{X};S= h; \text{compliers})\\
&=\mathbb{E}[Y(Z=1) - Y(Z=0) | S = h; \mathbf{X}].\\
\end{aligned}
$$
The bounds of $CATE(\mathbf{X};S= NI)$ are calculated by applying covariates $\mathbf{X}$ from the NI trial to the above functions derived from the historical trial. The partial estimators of ITT effects are [-0.024, -0.019], [-0.020, -0.016], [-0.017, -0.014] when $CC_{P}(\mathbf{X})$ = 0, 0.05, and 0.1.



is treated as a sensitive function whose value is in $\{0, 0.05, 0.1\}$ as it is almost impossible for participants to obtain TDF/FTC on their own.


HIV seroconversion endpoint for primary analysis is the outcome of interest. TDF/FTC is used as the active control in HPTN 084, while Cabotegravir is an experimental medication to be evaluated. In Partners PrEP Study, the actual treatment effect of active control versus placebo could be estimated. We restrict our analysis to the participants with complete information in HPTN 084 and Partners PrEP Study. \textcolor{blue}{In all, 415 participants are enrolled in HPTN 084 study and 1080 participants are enrolled in Partners PrEP Study.} We define compliers as the participants whose TDF/FTC pill taking rates $> 90\%$ and the compliance rate is 0.728 in Partners PrEP Study. While in HPTN 084, compliers are defined as the participants who were tested drug concentration larger than zero for every test interval, and the compliance rate is 0.383. \textcolor{red}{Will update to pill counts.}

\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
  \hline \\ [-0.8em]
  &\multicolumn{3}{c}{HPTN 084} &&\multicolumn{3}{c}{Prep}\\ \\ [-0.8em] \cline{2-4}\cline{6-8}
  
  &\multirow{4}{*}{\begin{tabular}{c}\textbf{Compliers +} \\ \textbf{Always takers} \\($\mathbb{E}[D(Z=1)]$)\end{tabular}}
  & \multirow{4}{*}{\begin{tabular}{c}\textbf{Always takers} \\   \\($\mathbb{E}[(Z=0)]$)\end{tabular}}
  &\multirow{4}{*}{\begin{tabular}{c}\textbf{Compliers} \\ \textbf{ } \\($\mathbb{E}[D(Z=1)] - E[D(Z=0)]$)\end{tabular}} &
  &\multirow{4}{*}{\begin{tabular}{c}\textbf{Compliers +} \\ \textbf{Always takers} \\($\mathbb{E}[D(Z=1)]$)\end{tabular}}
  & \multirow{4}{*}{\begin{tabular}{c}\textbf{Always takers} \\   \\($\mathbf{E}[D(Z=0)]$)\end{tabular}}
  &\multirow{4}{*}{\begin{tabular}{c}\textbf{Compliers} \\ \textbf{ } \\($\mathbb{E}[D(Z=1)] - E[D(Z=0)]$)\end{tabular}}\\ \\ \\ \\
  
  \textbf{Rate} &  0.383  &  NA & NA  &&   0.728  &   0 & 0.728 \\
   \hline
\end{tabular}}
\caption{Compliance rate for HPTN 084 and Prep}
\label{tb: WHI baseline characteristics}
\end{table}

The intention-to-treat effects of TDF/FTC in HPTN 084 can be identified through the estimation of conditional compliance $CC(\mathbf{X}; S = NI)$ and conditional average treatment effect $CATE(\mathbf{X}; S = NI)$ using the decomposition equation $ITT(\mathbf{X}; S = NI) = CC(\mathbf{X}; S = NI) \cdot CATE(\mathbf{X}; S = NI)$ if we admit population follows Assumption 3 in HPTN 084. The conditional compliance $CC(\mathbf{X}; S = NI) =CC_{AC}(\mathbf{X}; S = NI) - CC_{P}(\mathbf{X}; S = NI)$, where $CC_{AC}(\mathbf{X}; S = NI)$ is directly estimated from the planned NI trial HPTN 084 by virtue of randomization of active control and $CC_{P}(\mathbf{X}; S = NI)$ is treated as a sensitive function whose value is in $\{0, 0.05, 0.1\}$ as it is almost impossible for participants to obtain TDF/FTC on their own. $CATE(\mathbf{X}; S = h)$ is drived from the historical trial Partners PrEP Study, which can be point identified utilizing the decomposition equation if Assumption 3 holds in Partners PrEP Study. The point estimators of ITT effects are -0.026, -0.022, and -0.019 when $CC_{P}(\mathbf{X}; S = NI)$ = 0, 0.05, and 0.1. 
